Unveiling the (in)consistencies among the galaxy stellar mass function, star formation histories, satellite abundances and intracluster light from a semi-empirical perspective

In a hierarchical, dark matter-dominated Universe, stellar mass functions (SMFs), galaxy merger rates, star formation histories (SFHs), satellite abundances, and intracluster light, should all be intimately connected observables. However, the systematics affecting observations still prevent universal and uniform measurements of, for example, the SMF and the SFHs, inevitably preventing theoretical models to compare with multiple data sets robustly and simultaneously. We here present our holistic semi-empirical model DECODE (Discrete statistical sEmi-empiriCal mODEl) that converts via abundance matching dark matter merger trees into galaxy assembly histories, using different SMFs in input and predicting all other observables in output in a fully data-driven and self-consistent fashion with minimal assumptions. We find that: 1) weakly evolving or nearly constant SMFs below the knee ($M_\star \lesssim 10^{11} \, M_\odot$) are the best suited to generate star formation histories aligned with those inferred from MaNGA, SDSS, GAMA, and, more recently, JWST; 2) the evolution of satellites after infall only affects the satellite abundances and star formation histories of massive central galaxies but not their merger histories; 3) the resulting SFR-$M_\star$ relation is lower in normalization by a factor of $\sim 2$ with respect to observations, with a flattening at high masses more pronounced in the presence of mergers; 4) the latest data on intracluster light can be reproduced if mass loss from mergers is included in the models. Our findings are pivotal in acting as pathfinder to test the self-consistency of the high-quality data from, e.g., JWST and Euclid.

==> backup_text.tex <==
\begin{comment}
    
    \subsection{Star formation}\label{sec_dream_star_form}
    \haoc{Section to be probably cut}
    
    Star formation plays an extremely important role in the evolution of central galaxies, as well as for satellites after the infall. In this Section we present the methodology we apply to account for star formation into the time evolution of galaxies.
    
    In the vast majority of the cases star formation histories are usually calculated by fitting the spectral energy distribution of galaxies. In this work we adopt a novel methodology that allows to extract the SFHs by subtracting the mass from mergers to the total mass growth of the galaxy. This technique in principle exploits the maximum amount of information from the input data and does not introduce any specific parametrization assumed a-priori.
    
	In full generality, the total stellar mass $M_*$ of any galaxy is grown up by both the \textit{in situ} star formation and the contribution from mergers, and it is decreased by the stellar mass loss. We assume that all the contribution to the total growth history that does not come from mergers (ex-situ processes) must be due to the in-situ star formation. Thus, the total stellar mass at a given time can be represented as the sum of the two contributions:
    \begin{equation}
        M_{*, {\rm tot}} (t) = M_{*, {\rm SFR}} (t) + M_{*, {\rm mer}}(t)
    \end{equation}
    with $M_{*, {SF}}$ being the star formation history (SFH), i.e. the mass accreted by the star formation process. The amount of stellar mass formed via star formation per unit time is given by the star formation rate (SFR). The information on the mass loss is encoded in the global mass loss rate (GMLR).
    
    In order to calculate the SFH, we adopt the approach proposed by \cite{leitner_2011}:
    \begin{equation}
        \dot M_{*, {\rm SF}} = {\rm SFR} (M_*, z) - {\rm GMLR} (t)
    \end{equation}
    Here, the GMLR is given by the convolution of the SFR with the mass loss fraction $f_{\rm loss}$ given by:
    \begin{equation}
        {\rm GMLR} (t) = \int_t^{+\infty} {\rm SFR} (t') \dot{f}_{\rm loss} (t' - t) dt'
    \end{equation}
    \begin{equation}
        f_{\rm loss} = C_0 \ln \bigg( \frac{t}{\lambda} +1 \bigg)
    \end{equation}
    where $t$ is the lookback time and we adopt the parameters from \cite{moster_2018}, i.e. $C_0 = 0.05$ and $\lambda = 1.4 \; {\rm Myr}$, assuming a \cite{chabrier_2003} initial mass function.
    
	\end{comment}
	    
	\begin{comment}
    \section{The MCMC implementation}\label{sec_mcmc_implementation}
    
    In order to estimate and constraint the SMHM relation's parameters related to each SMF considered within this work, we perform a series of MCMC explorations using the SMF itself as input. In this subsection, we describe the methodology we use for this analysis and the type of likelihood adopted.
    
    In particular, our recipe for the MCMC scans can be summarized as follows:
    \begin{enumerate}
        \item We choose a SMF derived from observation, denoted as $\phi_{\rm obs}(M_{*,i})$, as input for our scan (e.g. \cite{leja_2019}).
        \item We generate a DM haloes and subhaloes catalogue within a reasonably large volume via \dream.
        \item We extract the SMF by making use of the SMHM relation to assign stellar mass to dark matter.
        \item For each MCMC step, we update the parameters of the SMHM and make use of the \dream catalogue to predict the updated SMF, denoted as $\phi_{\rm pred}(M_{*,i})$.
        \item For each step we update the likelihood to compare the predicted SMF with the one from observation. We adopt the $\chi^2$ definition for the likelihood as follows:
        \begin{equation}
            \chi^2 = \sum_{M_{*,i}} \bigg( \frac{\phi_{\rm obs}(M_{*,i}) - \phi_{\rm pred}(M_{*,i})} { \sigma_{\phi {\rm , obs}} (M_{*,i})} \bigg)^2
        \end{equation}
        with $\sigma_{\phi {\rm , obs}} (M_{*,i})$ being the uncertainty on the observed SMF.
    \end{enumerate}
    
    In order to optimize the CPU resources, we divide the MCMC analysis into two rounds. In particular, we first explore the parameters space of the four parameters at $z=0$, i.e. $\{ M_0, N_0, \beta_0, \gamma_0 \}$ assuming flat priors, finding a first raw estimation. Then, we perform a complete MCMC scan over the entire 8 parameters space, assuming as prior for the set of parameters at $z=0$ the posterior extracted from the previous analysis, and flat prior on the parameters at $z>0$.
    
    Furthermore, we introduce a cut-off when the SMF falls below $10^{-5}\, {\rm Mpc}^{-3} {\rm dex}^{-1}$, since below that value the SMF is extremely steep and easily affected by statistical fluctuations. Therefore, we ignore this interval at all in the MCMC when computing the likelihood.
    \end{comment}
    
    
    
    \begin{comment}
	    
	    \subsection{DM halo mergers}\label{sec_app_DM_mergers}
	    
	    First of all, we focus our attention on the merging history of DM haloes. In particular, we dedicate particular effort on testing the capability of our model to reproduce the number of mergers, since it is a crucial feature for predicting the merging history as further step. For this purpose, we compute the merger rates, i.e. the actual number of mergers per unit time, and compare it against results already obtained from N-body simulations. We execute this check for the DM merger and thus consider DM-only N-body simulations.
	    
	    We study the evolution in time of the merger rates for different values of central halo mass, and we limit our investigation to mergers with mass ratio $ f = M_{\rm h, sat} / M_{\rm h, cen} $ greater than $0.25$. In traditional statistical empirical models, the merger rate within a given redshift and therefore time bin $[t, t+\mathrm dt]$ is computed by numerically integrating Equation (\ref{eq_delta_shmf}) from the mass ratio of interest to infinite (\citealt{grylls_paper2}):
	    \begin{equation}
	        \frac{\mathm dN}{\mathrm dt} (t, M_{\rm h, cen}) = \int_{M_{\rm h, cen} * f}^{+\infty} \delta \phi (t+t+\mathrm dt, M_{\rm h, cen}, M_{\rm h, sat}) \mathrm d M_{\rm h, sat}
	    \end{equation}
	    with $\phi$ being the SHMF and $f = 0.25$ in our case.
	    
	    In this work, we employ a new recipe for calculating the merger rate by doing it in a discrete fashion. More particularly, for each mass value $\log (M_{\rm h}/ M_\odot)$ we select a significant number of central haloes that lies in the bin $[ \log (M_{\rm h}/ M_\odot), \log (M_{\rm h}/ M_\odot) + 0.1]$. For each of these objects, a history of the subhaloes which have infalled is known along with their masses at the time of infall and the merging timescale. This allows us to precisely compute the epoch $z_{\rm merge}$ at which the full merging occurs for each subhalo and, therefore, to count the real number of mergers that took place throughout the halo evolution history according to the recipe already described in Section \ref{sec_dream_evo_surv}. As additional remark, we stress that we neglect all the contributions from higher order mergers and restrict our exploration to first order subhaloes, as their statistical significance has already been tested and discussed in Section \ref{sec_valid_sub_pop}.
	    
	    \begin{figure}
	        \includegraphics[width=\columnwidth]{Figures/merger_rates_v2.pdf}
	        \caption{Time evolution of the merger rates in units of $[{\rm Gyr}^{-1}]$ for four different central halo masses ($\log (M_{\rm h, cen} / M_\odot) = 11, \, 12, \, 13, \, 14$). The dash-dotted lines represent the results from \dream, and the shaded areas the results of the Millennium simulation from \cite{fakhouri_2010}. \rezac{Given that DREAM should have a higher computational efficiency, I think the referee might ask why the DREAM lines are noisier than Millennium. Is it because of low statistics in this particular plot? Or is there any other reason?} \haoc{The noise I think is due to statistics because we are counting each single merger, while Fakhouri's curves are plotted using an analytical equation}}
	        \label{fg_merger_rates}
        \end{figure}
	    
	    Results for the merger rates are shown in Figure \ref{fg_merger_rates}. The outputs from \dream are represented with the coloured dash-dotted lines for different parent halo masses. The resultant merger rates are compared with those extracted from the Millennium simulation in \cite{fakhouri_2010} (solid shaded area). \rezac{I think it would be useful to add a few sentences about how DREAM predictions of merger rate vs. redshift compares with the Millennium simulation. In particular, why the difference gets stronger for low redshifts? Looking carefully at Fig. 7, DREAM's merger rate is significantly different from the merger rate of Millennium at z~0. Is that due to ignoring higher order mergers? Or low statistics?} \haoc{Yes, sorry about that, the comments on the comparison are still missing as we are still trying to understand it, I need to discuss this with Francesco. What I can say now is that it shouldn't be due to low statistics at $z \sim 0$...}
	    
	    \end{comment}
	    
	    
	    
	    
	    %We discuss in Section \ref{sec_validation} the details of the SMF and HMF we utilize for the abundance matching and the output SMHM.
        %The resultant SMHM relations are shown in Figure \ref{fg_SMHM_AM_scatter_comparison} for different redshift and for both null and non-null 0.15 dex scatter. The inclusion of a scatter in the AM mostly keeps the low mass end of the SMHM unvaried. On the other hand, a non-zero scatter slightly impacts the high mass end, shifting its value to lower galaxy mass at fixed halo mass. In this work we adopt in our investigation only a zero scatter and work with all mean quantities. As future work, we will investigate models with different constant values of scatter, as well as mass-dependent and redshift-dependent scatters.
        
        %Throughout this work we mainly make use of the SMHM from \cite{grylls_paper2} calculated by fitting the PyMorph SMF from \cite{bernardi_2017}. We also show the impact of using a steeper SMF at the low mass end, taking as example the one from \cite{leja_2019}. We show the two SMFs in Figure %\ref{fg_SMFs_comparison}.
        
        %\begin{figure}
        %    \includegraphics[width=\columnwidth]{Figures/SMF_bern_leja_comparison.pdf}
        %    \caption{Comparison between the total SMF from \cite{bernardi_2017} and from \cite{leja_2019}. \haoc{not sure if this plot is essential}}
        %    \label{fg_SMFs_comparison}
        %\end{figure}
        
        
        %\begin{figure}
	    %    \includegraphics[width=\columnwidth]{Figures/fraction_ellipticals_STEEL_comparison.pdf}
	    %    \caption{Fraction of elliptical galaxies as function of the galaxy stellar mass. The dash-dotted lines represent the prediction from \dream for two values of redshift and using inputs from \cite{grylls_paper2}, and the solid lines the results from their work. The triangles represent the T-Type selected fraction of ellipticals from SDSS at $z=0.1$.}
	    %    \label{fg_frac_ellipt}
        %\end{figure}
        
	    %As a very first test, we check the capability of \dream to reproduce the prediction of \cite{grylls_paper2} on the fraction of ellipticals. For this reason, we make use of exactly the same input assumptions from their work, i.e. the SMHM which has been calculated by fitting the PyMorph SMF from \cite{bernardi_2017}, and the dynamical friction timescale of \cite{mccavana_2012} without any fudge factor correction.
	    
	    %We report in Figure \ref{fg_frac_ellipt} the results of this check along with the T-Type selection of the ellipticals fraction taken from the SDSS (Sloan Digital Sky Survey) experiment. In the low mass range our predictions both at redshift 0.1 and 1 are consistent with the prediction of \cite{grylls_paper2}. On the other hand, at the high mass end we predict a higher fraction of ellipticals with respect to \citetalias{grylls_paper2} at $z=0.1$. In particular, \citetalias{grylls_paper2} estimates that galaxies with mass above $10^{11.5} M_\odot$ have 80\% of probability to undergo a major mergers, while our work predicts that above $10^{11} \odot$ major mergers occur for mostly all galaxies within that mass interval. At $z=1$ we have a consistent prediction.
	    
	    
	    
	    
	    \begin{comment}
	    \subsection{Mergers and SFH}
        
	    First of all, we focus our attention on the mass accretion of galaxies coming both from the contribution of mergers and star formation.
        
	    As already described in Section \ref{sec_dream_star_form}, we assume that the total growth in mass of a galaxy is given by only the two components of mergers and the in-situ star formation process. In order to show the application of this model, we compute the accretion and star formation histories of galaxies of different masses.
	    \end{comment}
